Data Debugging with Shapley Importance over End-to-End Machine Learning Pipelines

Developing modern machine learning (ML) applications is data-centric, of which one fundamental challenge is to understand the influence of data quality to ML training -- "Which training examples are 'guilty' in making the trained ML model predictions inaccurate or unfair?" Modeling data influence for ML training has attracted intensive interest over the last decade, and one popular framework is to compute the Shapley value of each training example with respect to utilities such as validation accuracy and fairness of the trained ML model. Unfortunately, despite recent intensive interest and research, existing methods only consider a single ML model "in isolation" and do not consider an end-to-end ML pipeline that consists of data transformations, feature extractors, and ML training. We present DataScope (ease.ml/datascope), the first system that efficiently computes Shapley values of training examples over an end-to-end ML pipeline, and illustrate its applications in data debugging for ML training. To this end, we first develop a novel algorithmic framework that computes Shapley value over a specific family of ML pipelines that we call canonical pipelines: a positive relational algebra query followed by a K-nearest-neighbor (KNN) classifier. We show that, for many subfamilies of canonical pipelines, computing Shapley value is in PTIME, contrasting the exponential complexity of computing Shapley value in general. We then put this to practice -- given an sklearn pipeline, we approximate it with a canonical pipeline to use as a proxy. We conduct extensive experiments illustrating different use cases and utilities. Our results show that DataScope is up to four orders of magnitude faster over state-of-the-art Monte Carlo-based methods, while being comparably, and often even more, effective in data debugging.

==> approach__OLD.tex <==
% !TEX root = datascope.tex

\begin{figure}
\centering
\includegraphics[width=0.4\textwidth]{figures/datascope.pdf}
\vspace{-1.5em}
\caption{Use DataScope for Data Debugging}
\label{fig:datascope}
\end{figure}

\section{DataScope}

We present \sysname, a data debugging and understanding approach for end-to-end ML pipelines. \sysname takes the following three inputs: (1)~a training set, (2)~a pre-defined utility (e.g., validation accuracy), and (3)~a \texttt{sklearn} pipeline, and outputs the {\em Shapley value} for each training example. \ssc{I think we should generalise this definition to talk about multiple inputs and pipeline mixing relational operations with estimator/transformer pipelines}

In the following, we describe \sysname's overall architecture and formally define the core technical problem of this work (Section~\ref{sec:approach-problem}). Next, we summarize the key enabling theoretical results in Section~\label{sec:approach-ptime} which demonstrate that we can compute Shapley values efficiently in PTIME for a large family of pipelines that we refer to as {\em canonical pipelines}. Last not but least, we describe our current strategies to approximate a given \texttt{sklearn} pipeline to a canonical pipeline in Section~\ref{sec:approach-approx}, and discuss our rationales behind such an approximation.

\vspace{-0.5em}
\subsection{Overview and Core Technical Problem}
\label{sec:approach-problem}

Figure~\ref{fig:datascope} illustrates the interaction between \sysname and a user on a toy example. The input of \sysname is a standard \texttt{sklearn} program (line 1-18) in which the user loads data (line 2-3), constructs an end-to-end pipeline consisting both feature extractors and an ML model (line 5-12), trains this pipeline(line 15), and tests its quality (line 18). \ssc{Let's use a more interesting pipeline with a join, a filter and a ColumnTransformer for multiple features}

\vspace{-0.5em}
\paragraph*{\underline{Data Debugging and 
Understanding as Data Importance}}

In real-world ML, one often encounters data-related problems in the input training set (e.g., wrong labels, outliers, biased samples) that leads to sub-optimal quality of the user's model.\ssc{cite deequ, validation paper from Google} The goal of \sysname is to facilitate the process of improving the data quality of the training set via efficient data debugging and data understanding. As illustrated in previous work~\citeX, many data debugging and understanding problems hinge on the following  fundamental question, which \sysname addresses: 
\begin{quote}
\em Which data examples in the training set are most important for the model utility ?
\end{quote}

A common approach, on which we also base our work, is to model this problem as computing the {\em Shapley value} of each data example as a measure of its importance to a model. This core functionality of \sysname is illustrated at line 24-28 in Figure~\ref{fig:datascope}, which assigns an importance value each training example. We illustrate several use cases of how these importance values can be used, including label denoising, data summarization,
and fairness debugging in Section~\refX. Note that Shapley values have been applied to a wide range use cases~\citeX. \ssc{cite XAI work which also heavily relies on Shapley values}

\paragraph*{\underline{Formal Definitions}}

\ssc{I think we need a more general definition here. I would suggest that a pipeline $f$ maps a set of relational inputs $\mathcal{D}_{{tr}_1},\dots,\mathcal{D}_{{tr}_k}$ (in star schema?) to the numerical inputs $\{z_i = (x_i, y_i)\}_{i \in [n]} $ for the model $\mathcal{A}$. I think this formulation makes it easier to think about joins in the pipeline, and make it clear what the challenges of including the pipeline in the picture are.}

We formally define the core technical problem addressed by \sysname as follows. Let $\mathcal{D}_{tr}=\{z_i = (x_i, y_i)\}_{i \in [n]}$ be a training set, let $f$ denote a feature extraction pipeline and $\mathcal{A}$ be a ML training algorithm. After feature extraction and training, we obtain an ML model:  
\[
\mathcal{A} \circ f (\mathcal{D}_{tr}).
\]
Note that in Figure~\ref{fig:datascope}, $\mathcal{A} \circ f $ corresponds to the pipeline \texttt{pipe}~(Line 7-12). \ssc{We could nest the feature encoding operations into their own pipeline to make this clearer.} We can measure the ``performance'' of this model in various ways, e.g., via validation accuracy and a fairness metric \ssc{cite survey paper for fairness metrics here}. Let $\mathcal{D}_{val}=\{\tilde{z}_i = (\tilde{x}_i, 
\tilde{y}_i)\}_{i \in [m]}$ \ssc{This should also be a set of relational inputs} be a given validation set. Based on this, we define a utility function $u$, which measures the performance of this trained end-to-end pipeline:
\[
u (\mathcal{A} \circ f (\mathcal{D}_{tr}), f(\mathcal{D}_{val})) \mapsto [0, 1].
\]
In this paper, we will focus on what we refer to as \textcolor{red}{\textit{additive utilities}}, which cover the most important set of utilities functions in practice (e.g., validation loss, validation accuracy, many different fairness metrics). We say 
an utility function is \textit{additive} if:
\[
u (\mathcal{A} \circ f (\mathcal{D}_{tr}), f(\mathcal{D}_{val}))
= 
\sum_{\tilde{z} \in \mathcal{D}_{val}}
   u (\mathcal{A} \circ f (\mathcal{D}_{tr}), f(\{\tilde{z}\})).
\]

\ssc{Maybe give an example for non-intuitive cases, such as fairness measures}

For the simplicity of the notation, we use the following notation in cases where the validation set $\mathcal{D}_{val}$ is clear from the context:

\[
u \circ \mathcal{A} \circ f (\mathcal{D}_{tr}) := u (\mathcal{A} \circ f (\mathcal{D}_{tr}), f(\mathcal{D}_{val}))
\]

\paragraph*{\underline{Shapley Value}}

The Shapley value, denoting the importance of a training example $z_i$, is defined as
\[
\phi_i = \frac{1}{n} \sum_{S \subseteq \mathcal{D}_{tr} \backslash \{z_i\}} {n - 1 \choose |S|}^{-1} \left( 
    u \circ \mathcal{A} \circ f (S \cup \{z_i\}) -
    u \circ \mathcal{A} \circ f (S) 
\right). 
\]
Intuitively, the {\em importance} of a data example $z_i$ over a subset of 
training examples $S \subseteq \mathcal{D}_{tr} \backslash \{z_i\}$
is measured as the difference of the utility $u \circ \mathcal{A} \circ f (S \cup \{z_i\})$ \textit{with} $z_i$ to the utility $u \circ \mathcal{A} \circ f (S)$ \textit{without} the specific example $z_i$. The Shapley value takes the average of all such possible subsets $S \subseteq \mathcal{D}_{tr} \backslash \{z_i\}$, which allows it to have a range of desired properties that significantly benefit data debugging tasks~\citeX. \ssc{Name and discuss these benefits briefly}

\paragraph*{\underline{Challenges and Monte Carlo Baselines}}
%
\ssc{Parts of this could be moved to preliminaries}
All previous research focuses on the scenario in which there is no feature
extraction pipelines (i.e., $f(D) \mapsto D$); \ssc{If we assume that the pipeline transforms relations into a matrix, then this statement becomes even stronger} even in this case, computing Shapley values is tremendously hard since its complexity  for general ML models is \texttt{\#P}-hard.
Previous work accommodates this computational challenge in two different ways:
\begin{enumerate}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt,topsep=0pt, leftmargin=*]
\item {\bf Monte Carlo Shapley}: One line of efforts tries to estimate Shapley values with Markov Chain Monte Carlo (MCMC)-based techniques. This includes vanilla Monte Carlo sampling~\citeX, group testing~\citeX, and Truncated Monte Carlo~\citeX sampling. \ssc{We should describe these a bit in one sentence}
\item {\bf KNN Shapley}: 
Even the most efficient  Monte Carlo-based methods need 
to train multiple ML models (in order to evaluate $\mathcal{A}$ multiple times on different subsets of the features) and thus do not scale to datasets of even of modest size \ssc{Add a reference for that}. As a consequence, an alternative line of research proposes to approximate the model $\mathcal{A}$ using a simpler proxy model. Specifically, previous work shows that 
Shapley values can be computed over K-nearest neighbors (KNN) classifiers
in PTIME~\citeX, and that leveraging these as a proxy is very effective in a various real-world scenarios~\citeX.
\end{enumerate}

In \sysname, we are facing an even harder problem
given the presence of a feature extraction pipeline. \ssc{Explain what exactly is harder!} Nevertheless, as a baseline, it is important to
realize that all Monte Carlo-based approaches~\citeX can be 
directly extended to support \sysname. This is because most, of not all, Monte Carlo-based approaches model training as a {\em black box function} and thus, can be used directly to handle an end-to-end pipeline:

$\mathcal{A} \circ f$.

\ssc{Is this really the case? If the pipeline joins multiple inputs, we will only get the Shapley values for the join result, right?}

\paragraph*{\underline{Core Technical Problem}}
Despite the existence of a Monte Carlo baseline \ssc{Again, will this baseline produce correct results for the fork and join cases?},
as we will see in Section~\refX,
it suffers when it comes to 
scalability and speed --- in 
our experiments, it is not uncommon for 
such a Monte Carlo baseline to take 
1 hour to compute Shapley value 
on even a small dataset with only 1000 examples!
To bring data debugging and understanding
into practice, we are in dire needs
for a more efficient and scalable alternative.

Without a feature extraction pipeline, 
using KNN as a proxy model has been shown 
to be orders of magnitude faster
than its Monte Carlo counterpart~\citeX
while being equally, if not more, 
effective on many applications~\citeX. \ssc{List one or two of these applications}
{\em Can we similarly use a KNN classifier 
as a proxy for \sysname}?

\ssc{It might make sense to split up these section into two sections, a problem statement (until here) and then a follow up section for the approximation of pipelines}



\subsection{PTIME KNN Shapley for canonical Pipelines}
\label{sec:approach-ptime}

Extending KNN Shapley to an end-to-end 
ML pipeline is a far more challenging
problem compared with Monte Carlo-based approach.
Today's KNN Shapley algorithm heavily relies
on the structure of the KNN classifier.
The presence of a feature extraction pipeline 
will drastically change the underlying
algorithm and time complexity --- in fact,
for many feature extraction pipelines,
we expect that Shapley is \texttt{\#P}-hard
even for KNN classifiers!

\ssc{Give an intuition why this is the case. Is is related to global aggregations in these pipelines?}


The key technical contribution of this paper is a novel algorithmic framework which covers a large sub-family of ML pipelines whose KNN Shapley can be computed in PTIME. We call these pipelines \textit{canonical pipelines}.


\begin{theorem}
Let $\mathcal{D}_{tr}$ be a training set of $n$ examples, $f$ be a feature extractor over $\mathcal{D}_{tr}$, and  $\mathcal{A}_{knn}$ be a $K$-nearest neighbor classifier. 
\textcolor{red}{If $f$ can be expressed as 
an Additive Decision Diagram (ADD) with polynomial
size, then computing}
\begin{small}
\[
\phi_i = \frac{1}{n} \sum_{S \subseteq \mathcal{D}_{tr} \backslash \{z_i\}} {n - 1 \choose |S|}^{-1} \left( 
    u \circ \mathcal{A}_{knn} \circ f (S \cup \{z_i\}) -
    u \circ \mathcal{A}_{knn} \circ f (S) 
\right)
\]
\end{small}
is in \texttt{PTIME} for all additive utilities $u$.
\label{theorem:main}
\end{theorem}

\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{figures/patterns.pdf}
\vspace{-2em}
\caption{Three types of canonical pipelines over which 
Shapley values can be computed in PTIME.}
\label{fig:patterns}
\end{figure}

This theorem provides a sufficient condition under which
we can compute Shapley values for KNN classifiers 
over ML pipelines. We can instantiate this general framework with  concrete types of feature extraction pipelines.
We leave the details of these highly non-trivial technical results to Section~\refX, summarize three types of
canonical pipelines whose Shapley value can be computed in PTIME, and illustrate them in Figure~\ref{fig:patterns}.

What is interesting, especially to the data management 
community, is that the time complexity 
of computing KNN Shapley over feature
extraction pipeline $f$ heavily relies on the
\textit{data provenance}~\citeX 
of this specific ML pipeline $f$:

\vspace{0.5em}
{\bf \em Map pipelines} are a subfamily of pipeline that
satisfy the condition in Theorem~\ref{theorem:main}, in which
the feature extraction $f$ has the following property: each 
input training example $z_i$ is transformed into a unique 
output training example $z_i'$ with an arbitary tuple-at-a-time
transformation function $h_f$:
\[
z_i \mapsto z'_i = h_f(z_i)
\]
\ssc{We could mention the structure of the provenance polynomials here}

\vspace{0.5em}
{\bf \em Fork pipelines} are a superset of Map pipelines which
requires that for each output example $z_j'$, there exists a \textit{unique} 
input example $z_i$, such that 
$z_j'$ is generated by applying an arbitrary tuple-at-a-time
transformation function $h_f$ over $z_i$: $z_j' = h_f(z_i)$. As illustrated in Figure~\ref{fig:patterns}(b),
the output examples $z_1'$ and $z_2'$ are both 
generated by input example $z_1$. Fork pipelines
also satisfy the condition in Theorem~\ref{theorem:main}.

\ssc{We could mention the structure of the provenance polynomials here}

\vspace{0.5em}
{\bf \em One-to-many Join} is illustrated in 
Figure~\ref{fig:patterns}(c). 
XXX \\
XXX \\
XXX \\
XXX \\
XXX \\
XXX \\
XXX 

\ssc{I think we need to extend the definition of the pipelines to handle join pipelines, we need to be able to have multiple inputs and joins in the definition}

\subsection{Approximating Real-world Pipelines}
\label{sec:approach-approx}

\ssc{I think we can rewrite this to be more general if we talk about ML pipelines as a combination of relational operations with estimator/transformer pipelines, which also covers SparkML and some parts of TFX}

Given an \texttt{sklearn} pipeline 
\[
\texttt{pipe} := (\mathcal{A}, f)
\]
in practice, often these do not directly give us a canonical pipeline whose Shapley value can be computed
in PTIME. \ssc{Explain why} In \sysname, a key operation is to 
\textit{approximate} this pipeline into a canonicals pipeline, in two ways.

\paragraph*{\underline{Approximate $\mathcal{A}$}}
The first approximation follows various previous efforts summarised as KNN Shapley before, and has been shown to work well, if not better,
in a diverse range of scenarios~\citeX.
In this step, we approximate the pipeline's ML model with a KNN classifier
\[
\mathcal{A} \mapsto \mathcal{A}_{knn}.
\]

\paragraph*{\underline{Approximate $f$}}
In terms of the feature extraction pipeline, 
it becomes more complex. In practice, we see that a given feature extraction \textit{pipeline} consists of a sequence of 
feature extraction \textit{operators}, e.g., \texttt{MinMaxScaling}, \texttt{PCA}, \texttt{TFIDF}. Each of these operators can often be expressed with a \texttt{fork-reduce} pattern over the data:
\[
op(\mathcal{D}) = \texttt{fork}(\texttt{reduce}(\mathcal{D}), \mathcal{D}).
\]

\ssc{I think we should rewrite this to talk about the estimator/transformer abstraction to make it more general. The transformer is the map, and the estimator computes a global statistic over the data to generate a ``fitted'' transformer, which is the reduce part of things here}

During the \texttt{reduce} step, operators compute some global statistics over the dataset --- in \texttt{MinMaxScaling} it computes the \texttt{Min} and \texttt{Max} values and in \texttt{TFIDF} it computes the \texttt{IDF} value. During the \texttt{fork} step, operators transform the input dataset using these global statistics --- in \texttt{MinMaxScaling} it normalizes  each data example with the computed \texttt{Min} and \texttt{Max}.

The \texttt{reduce} step is often the key reason that a feature extraction pipeline cannot have PTIME Shapley computation. \ssc{Explain why} Fortunately, we also observe that they are 
relatively stable given different subset  of the data, especially what we want to compute is the \textit{difference}
when a single example is added or removed. \ssc{We should mention that we experimentally validate this later}
One approximation that we conduct is to let the \texttt{reduce}
component to take only as input the whole dataset: \ssc{in sklearn terms, we reuse the transformer generated by fitting the estimator on the whole dataset. We do the same thing in mlinspect btw.}
\[
op(\mathcal{D}) = \texttt{fork}(\texttt{reduce}(\mathcal{D}), \mathcal{D}) \mapsto 
op^*(\mathcal{D}) = \texttt{fork}(\texttt{reduce}(\mathcal{D}_{tr}), \mathcal{D})
\]

\ssc{I think this should be map not fork, sklearn pipelines cannot change the output size}

Once all operators $op$ in an input pipeline are transformed into their approximate variant $op^*$, a large majority of realistic pipelines become canonical pipelines of a \texttt{fork} pattern. \ssc{I think this should be map!}

XXX \\
XXX \\
XXX 

\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{figures/coverage.pdf}
\vspace{-2em}
\caption{\textcolor{red}{A dominating majority of real-world ML pipelines~\citeX
have a canonical pipeline of map-fork pattern.}}
\label{fig:coverage}
\end{figure}

\paragraph*{\underline{Statistics of Real-world Pipelines}}
Figure~\ref{fig:coverage} illustrates a case study
that we conducted over 500K real-world pipelines
provided by Microsoft~\citeX. We see that \\
XXX \\
XXX \\
XXX \\
XXX \\
XXX \\
XXX 

\ssc{I can help plotting this if you give the data or the statistics}

\paragraph*{\underline{Discussion: What if These Two Approximations Fail?}}
Computing Shapley values for a generic pipeline
$(\mathcal{A}, f)$ is \#P-hard, and by
approximating it into
$(\mathcal{A}_{knn}, f^*)$, we obtain an 
efficient PTIME solution. This drastic improvement
on complexity also means that \textit{we should
expect that there exist scenarios under which
this $(\mathcal{A}, f) \mapsto (\mathcal{A}_{knn}, f^*)$
approximation is not a good approximation.}

\vspace{0.3em}
{\em How often would this failure case happen in
practice?} 
When the training set is reasonably large, 
as illustrated in many previous studies focusing on the KNN proxy, we are relatively confident that the $\mathcal{A} \mapsto \mathcal{A}_{knn}$ approximation should work well in most practical scenarios \ssc{this sounds a bit vague}, and only fails when we are relying on some very strong global 
properties that KNN does not model. \ssc{such as?} 
As for the $f \mapsto f^*$ approximation, we expect the failure cases to be even more rare, especially when the training set 
is reasonably large. \ssc{how large is that?}
These two beliefs are empirically verified in our extensive experiments in Section~\refX, and backed up by various previous empirical results on KNN Shapley~\citeX.

\vspace{0.3em}
{\em What should we do when such a failure case
happen?} Nevertheless, we should expect 
such a failure case can happen in practice.
In this case, we will resort to the Monte Carlo baseline,
which will be orders of magnitude slower, but
should provide a backup alternative in this case.
It is an exciting future direction to further 
explore the limitations of both approximations and 
develop more efficient Monte Carlo methods. \ssc{Does this work for join pipelines?}

==> framework-backup.tex <==
% !TEX root = datascope.tex

\section{Algorithm Framework: KNN Shapley Over Data Provenance}
\label{sec:framework}

In this section we describe our method for efficiently computing the Shapley value as defined in \autoref{eq:shap-basic} over the K-Nearest Neigbor accuracy utility as defined in \autoref{eq:knn-acc-definition}. To start off, we need to transform the original Shapley value formula to better fit our setting where the set of players $\mathcal{X}$ corresponds to variables associated with source data tuples. These tuples then get passed through a feature processing pipeline $f$ to produce a training dataset $\mathcal{D}_{tr}$. According to semantics described in \autoref{sec:end-to-end-ml-pipelines}, each dataset represents a set of candidate datasets, each one defined by a distinct value assignment $v \in \mathcal{V}_{\mathcal{X}}$.

Therefore, we replace the sum over sets $S$ of active players from \autoref{eq:shap-basic} with a sum over value assignments. Thus we obtain the following definition of the Shapley value for source tuple associated with variable $x_i$:
\begin{equation} \label{eq:shap-pipeline}
\resizebox{0.9\hsize}{!}{$
    \varphi_i = \frac{1}{|\mathcal{X}|} \sum_{v \in \mathcal{V}_{\mathcal{X} \setminus \{ x_i \}}}
    %\binom{N-1}{|\mathrm{supp}(v)|}^{-1}
    %\frac{\left( u(f(\mathcal{D}[v[x_i \gets 1]])) - u(f(\mathcal{D}[v]))\right)}
    \frac{u(\mathcal{D}_{tr}[v[x_i \gets 1]]) - u(\mathcal{D}_{tr}[v[x_i \gets 0]])}
    {\binom{|\mathcal{X}|-1}{|\mathrm{supp}(v)|}}
$}
\end{equation}
In the above formula, the notational expression $v[x_i \gets X]$ represents the same value assignment as $v$, except that we enforce that $v(x_i) = X$ for some constant $X$. Also, the support $\mathrm{supp}(v)$ of a value assignment $v$ is a subset of $\mathcal{X}$ of variables that are assigned the value $1$ according to $v$.

By observing \autoref{eq:shap-pipeline} we can notice that the time complexity is still exponential in the number of variables. Our goal in this section is to compute $\varphi_i$ in polynomial time. In \autoref{sec:shapley-with-oracle} we describe a strategy to partition that large sum and push the exponential computation in a so-called \emph{counting oracle}. Then in \autoref{sec:oracle-with-add} we describe a method of computing that oracle using decision diagrams described in \autoref{sec:additive-decision-diagrams}. We then show in \autoref{sec:add-for-pipeline} that polynomial-time algorithms are indeed possible for the classes of feature processing pipelines described in \autoref{sec:representing-pipelines}. Finally, in \autoref{sec:special-case-1nn} we describe some further optimizations for the special case of the KNN model when $K=1$.

\ww{Given that all this section is about computing the Shapley value over the pipeline lineage, I think we perhaps can have a summary subsection first to give a diagram and a running example. We can then follow the same pattern in each of Sections 5.1, 5.2, and 5.3 to focus on intuition and examples, and defer the technical details to the full version.}




\subsection{PTIME Shapley Algorithm with PTIME Counting Oracle} \label{sec:shapley-with-oracle}

Starting from \autoref{eq:shap-pipeline} and plugging in the KNN accuracy utility defined in \autoref{eq:knn-acc-definition}, we can augment the expression for computing $\varphi_i$ as such:
\begin{equation}
    % \resizebox{0.9\hsize}{!}{$
    \begin{split}
        \varphi_i = \frac{1}{N}
        \sum_{v \in \mathcal{V}_{\mathcal{X} \setminus \{ x_i \}}}
        \sum_{\alpha=1}^{N}
            & \mathbbm{1} \{ \alpha = |\mathrm{supp}(v)| \}
            \binom{N-1}{\alpha}^{-1} \\
        \cdot \sum_{t, t' \in \mathcal{D}_{tr}}
            & \mathbbm{1} \{ t = \mathrm{top}_K \mathcal{D}_{tr}[v[x_i \gets 0]] \} \\
            \cdot & \mathbbm{1} \{ t' = \mathrm{top}_K \mathcal{D}_{tr}[v[x_i \gets 1]] \} \\
        \cdot \sum_{\gamma, \gamma' \in \Gamma}
            & \mathbbm{1} \{ \gamma = \mathrm{tally}_{t} \mathcal{D}_{tr}[v[x_i \gets 0]] \} \\
            \cdot & \mathbbm{1} \{ \gamma' = \mathrm{tally}_{t'} \mathcal{D}_{tr}[v[x_i \gets 1]] \} \\
            \cdot & \mathrm{acc}_{\Delta} (\gamma, \gamma')
    \end{split}
    % $}
    \label{eq:shap-transform-1}
\end{equation}
Here, the innermost accuracy gain function is formally defined as
$\mathrm{acc}_{\Delta} (\gamma, \gamma') := \mathrm{acc}(\gamma') - \mathrm{acc}(\gamma)$
where
$\mathrm{acc}(\gamma) := \mathbbm{1}\{ \ell(t_v) = \mathrm{argmax}_{c \in C} \gamma \}$.
The correctness of \autoref{eq:shap-transform-1} comes from the observation that for any distinct $v \in \mathcal{V}_{\mathcal{X} \setminus \{ x_i \}}$, there is a unique solution to all predicates. Namely, there is a single $t$ that is the $K$-th most similar tuple when $v(x_i)=0$, and similarly for $t'$ when $v(x_i)=1$. Given those \emph{boundary tuples} $t$ and $t'$, the same goes for the \emph{tally vectors} $\gamma$ and $\gamma'$ which are unique for given $\mathcal{D}_{tr}[v[x_i \gets 0]]$ and $\mathcal{D}_{tr}[v[x_i \gets 1]]$ respectively. \todo{Clarify better.}

If we reshufle the sums in \autoref{eq:shap-transform-1} by pushing them outside, we can isolate the sum over value assignments, along with all the predicates to obtain the expression for the \emph{counting oracle} which is defined as follows:
\begin{equation}
    \resizebox{0.9\hsize}{!}{$
    \begin{split}
        \omega_{t, t'} (\alpha, \gamma, \gamma') :=
        \sum_{v \in \mathcal{V}_{\mathcal{X} \setminus \{ x_i \}}}
        \cdot & \mathbbm{1} \{ \alpha = |\mathrm{supp}(v)| \} \\
        \cdot & \mathbbm{1} \{ t = \mathrm{top}_K \mathcal{D}_{tr}[v[x_i \gets 0]] \} \\
        \cdot & \mathbbm{1} \{ t' = \mathrm{top}_K \mathcal{D}_{tr}[v[x_i \gets 1]] \} \\
        \cdot & \mathbbm{1} \{ \gamma = \mathrm{tally}_t \mathcal{D}_{tr}[v[x_i \gets 0]] \} \\
        \cdot & \mathbbm{1} \{ \gamma' = \mathrm{tally}_t \mathcal{D}_{tr}[v[x_i \gets 1]] \}
    \end{split}
    $}
    \label{eq:counting-oracle}
\end{equation}

By isolating the exponential part of the computation into a counting oracle $\omega_{t, t'}$, we can obtain the following simplified formula for computing the Shapley value:
\begin{equation}
    \resizebox{0.9\hsize}{!}{$
        \varphi_i = \frac{1}{N}
        \sum_{t, t' \in \mathcal{D}_{tr}}
        \sum_{\alpha=1}^{N}
        \binom{N-1}{\alpha}^{-1}
        \sum_{\gamma, \gamma' \in \Gamma}
        \mathrm{acc}_{\Delta} (\gamma, \gamma')
        \omega_{t, t'} (\alpha, \gamma, \gamma')
    $}
    \label{eq:shap-main}
\end{equation}
In the above formula, we can notice that all sums iterate over a number of elements that is linear in the size of data $|\mathcal{D}_{tr}|$ and the number of variables $|\mathcal{X}|$. Thus, it becomes clear that computing the above expression in polynomial time is conditioned upon being able to compute the oracle $\omega_{t, t'}$ in polynomial time. This observation is summarized in the following theorem:
\begin{theorem} \label{thm:counting-oracle}
    If each counting oracle $\omega_{t, t'}$ can be computed in polynomial time with respect to the size of data, then the Shapley value $\varphi_i$ for the KNN accuracy utility can also be computed in polynomial time with respect to the size of data.
\end{theorem}

\subsection{PTIME Counting Oracle using PSPACE ADD's} \label{sec:oracle-with-add}

Our goal is to efficiently compute the counting oracle $\omega_{t, t'}$ as defined in \autoref{eq:counting-oracle}. Our approach is to model this problem using an Additive Decision Diagram (ADD). ADD's represent Boolean functions $\phi : \mathcal{V}_{\mathcal{X}} \rightarrow \mathcal{E} \cup \infty$ that map value assignments $v \in \mathcal{V}_{\mathcal{X}}$ to elements of some set $\mathcal{E}$ or to a special invalid element $\infty$. Since we are allowed to design the set $\mathcal{E}$ based on our problem, we will define it as $\mathcal{E} := \{1,...,|\mathcal{X}|\} \times \Gamma \times \Gamma$ where $\Gamma$ is the set of label tally vectors defined in $\autoref{eq:tally-vector-set}$. We introduce our Boolean function $\phi_{t, t'} : \mathcal{V}_{\mathcal{X}}[x_i=0] \rightarrow \mathbbm{N}$ which we formally define as follows:

\begin{equation} \label{eq:oracle-add-function}
    % \resizebox{0.9\hsize}{!}{$
    \begin{split}
        \phi_{t, t'}(v) &:= \begin{cases}
            \infty,     & \mathrm{if} \ t \not\in \mathcal{D}\big[v[x_i \gets 0]\big], \\
            \infty,     & \mathrm{if} \ t' \not\in \mathcal{D}\big[v[x_i \gets 1]\big], \\
            (\alpha, \gamma, \gamma' ),     & \mathrm{otherwise} \\
        \end{cases} \\
        \alpha &:= |\mathrm{supp}(v)| \\
        \gamma &:= \mathrm{tally}_{t} \mathcal{D}\big[v[x_i \gets 0]\big] \\
        \gamma' &:= \mathrm{tally}_{t'} \mathcal{D}\big[v[x_i \gets 1]\big]
    \end{split}
    % $}
\end{equation}
If we can construct an ADD with a root node $n_{t, t'}$ that computes $\phi_{t, t'}(v)$ exactly as defined in the above expression, then the following equality holds:
\begin{equation}
    \omega_{t, t'} (\alpha, \gamma, \gamma') = \mathrm{count}_{(\alpha, \gamma, \gamma')} (n_{t, t'})
\end{equation}
Given that in \autoref{sec:additive-decision-diagrams} we saw that the complexity of model counting is $O(|\mathcal{N}| \cdot |\mathcal{E}|)$ and since the size of $\mathcal{E}$ is polynomial in the size of data, we can derive the following theorem:
\begin{theorem} \label{thm:decision-diagram}
If we can represent the $\phi_{t, t'}(v)$ in \autoref{eq:oracle-add-function} with an ADD of size polynomial in $|\mathcal{X}|$ and $|\mathcal{D}_{tr}|$, we can compute the counting oracle $\omega_{t, t'}$ in time polynomial of $|\mathcal{X}|$ and $|\mathcal{D}_{tr}|$.
\end{theorem}

\subsection{Constructing PSPACE ADD's for ML Pipelines} \label{sec:add-for-pipeline}

\begin{algorithm}[t!]
    \scriptsize
    \caption{Compiling a provenance-tracked dataset into ADD.} \label{alg:compile-dataset-to-add}
    \begin{algorithmic}[1]
    
    
    \Function{CompileADD}{}
    % $\omega$, $\mathcal{D}_{tr}$, $\mathcal{X}$, $x_i$, $K$, $C$
    
    \Inputs
    \Input{$\mathcal{D}$, provenance-tracked dataset;}
    \Input{$\mathcal{X}$, set of variables;}
    \Input{$t$, boundary tuple;}
    \Outputs
    \Output{$\mathcal{N}$, nodes of the compiled ADD;}
    
    \Begin
    
    \State $\mathcal{N} \gets \{\}$
    \State $\mathcal{P} \gets \{ (x_1, x_2) \in \mathcal{X} \ : \exists t \in \mathcal{D}, x_1 \in p(t) \ \wedge \ x_2 \in p(t) \}$
    \State $\mathcal{X}_{L} \gets $ \Call{GetLeafVariables}{$\mathcal{P}$} \label{alg:cmp:line:leaves}
    % \State $\mathcal{X}^{(1)}, \mathcal{X}^{(2)}, ..., \mathcal{X}^{(M)} \gets $ \Call{ConnectedComponents}{$\mathcal{P}$}
    % \For{$\alpha \in \mathrm{ConnectedComponents}(\mathcal{P})$}
    \For{$\mathcal{X}_{C} \in $ \Call{GetConnectedComponents}{$\mathcal{P}$}} \label{alg:cmp:line:conn-cmp}
        \State $\mathcal{N}' \gets $ \Call{ConstructADDTree}{$\mathcal{X}_C \setminus \mathcal{X}_L$} \label{alg:cmp:line:add-tree}
        
        \State $\mathcal{X}' \gets \mathcal{X}_C \setminus \mathcal{X}_L$
        % \State $\mathcal{N}' \gets \{\}$
        \State $\mathcal{D}' \gets \{ t' \in \mathcal{D} \ : \ p(t') \cup \mathcal{X}_C \neq \emptyset \}$
        \For{$v \in \mathcal{V}_{\mathcal{X}'}$}
            \State $\mathcal{N}_C \gets $ \Call{ConstructADDChain}{$\mathcal{X}_C \cap \mathcal{X}_L$}
            \For{$n \in \mathcal{N}_C$}
                \State $v' \gets v \cup \{ x(n) \rightarrow 1 \}$
                \State $a_H(n) \gets |\{ t' \in \mathcal{D}' \ : \ \mathrm{eval}_{v'} p(t') = 1 \ \wedge \ \sigma(t') \geq \sigma(t) \}|$
            \EndFor
            
            \State $\mathcal{N}' \gets $ \Call{AppendToADDPath}{$\mathcal{N}'$, $\mathcal{N}_C$, $v$} \label{alg:cmp:line:append-path}
        \EndFor
        \State $\mathcal{N} \gets $ \Call{AppendToADDRoot}{$\mathcal{N}$, $\mathcal{N}'$}
        
        % \For{$n \in \mathcal{N}$ \textbf{where} $n_L(n) = \boxdot$ \textbf{or} $n_H(n) = \boxdot$}
        % \EndFor
    \EndFor
    
    \For{$x' \in p(t)$}
        \For{$n \in \mathcal{N}$ \textbf{where} $x(n) = x'$}
            \State $a_L(n) \gets \infty$
        \EndFor
    \EndFor
    
    
    \Return $\mathcal{N}$
    
    \EndFunction
    
    \end{algorithmic}
\end{algorithm}

In this section we describe the procedure for constructing a ADD for a given dataset $\mathcal{D}$ made up of tuples that are annotated with provenance polynomials. The main procedure \textsc{CompileADD} is defined in \autoref{alg:compile-dataset-to-add}. Invoking \textsc{CompileADD}($\mathcal{D}$, $\mathcal{X}$, $t$) constructs an ADD with node set $\mathcal{N}$ that computes the following function:
\begin{equation} \label{eq:oracle-add-function-single}
    \phi_{t}(v) := \begin{cases}
        \infty,     & \mathrm{if} \ t \not\in \mathcal{D}[v], \\
        \mathrm{tally}_t \mathcal{D}[v]    & \mathrm{otherwise} \\
    \end{cases}
\end{equation}
%$\phi_{t}(v) := \infty, \ \mathrm{if} \ t \not\in \mathcal{D}[v]$, and $\phi_{t}(v) := \mathrm{tally}_t \mathcal{D}[v] \ \mathrm{otherwise}$.

To construct the function defined in \autoref{eq:oracle-add-function}, we need to invoke \textsc{CompileADD} once more by passing $t'$ instead of $t$ in order to obtain another diagram $\mathcal{N}'$. The final diagram is obtained according to the expression defined as $\mathcal{N}[x_i \gets 0] + \mathcal{N}'[x_i \gets 1]$. The size of the resulting diagram will still be bounded by $O(|\mathcal{D}|)$. \todo{Missing $\alpha$.}

We can now examine different types of ML pipelines and see how their structures are reflected onto the ADD's.

%\medskip \noindent \textbf{One-to-Many Join Pipelines.} 
\inlinesection{One-to-Many Join Pipeline}
In a \emph{star} database schema, this corresponds to a \emph{join} between a \emph{fact} table and a \emph{dimension} table, where each tuple from the dimension table can be joined with multiple tuples from the fact table. It can be represented by an ADD similar to the one in \autoref{fig:example-add-structure}. %Given this structure, we can derive the following corollary:

\begin{corollary}
For the $K$-NN accuracy utility and a one-to-many \emph{join} pipeline, which takes as input two datasets, $\mathcal{D}_F$ and $\mathcal{D}_D$, of total size $|\mathcal{D}_F| + |\mathcal{D}_D| = N$ and outputs a joined dataset of size $O(N)$, the Shapley value can be computed in $O(N^4)$ time.
\end{corollary}

%\medskip \noindent \textbf{Fork Pipelines.} 
\inlinesection{Fork Pipeline}
The key characteristic of a pipeline $f$ that contains only \emph{fork} or \emph{map} operators is that the resulting dataset $f(\mathcal{D})$ has provenance polynomials with only a single variable. This is due to the absence of joins, which are the only operator that results in provenance polynomials with a combination of variables. %We can use this observation to prove the following corollary:

\begin{corollary}
For the $K$-NN accuracy utility and a \emph{fork} pipeline, which takes as input a dataset of size $N$ and outputs a dataset of size $M$, the Shapley value can be computed in $O(M^2 N^2)$ time.
\end{corollary}

%\medskip \noindent \textbf{Map Pipelines.} 
\inlinesection{Map Pipeline}
A \emph{map} pipeline is similar to \emph{fork} pipeline in the sense that every provenance polynomial contains only a single variable. However, each variable now can appear in a provenance polynomial of \emph{at most} one tuple, in contrast to \emph{fork} pipeline where a single variable can be associated with \emph{multiple} tuples. This additional restriction results in the following corollary:

\begin{corollary}
For the $K$-NN accuracy utility and a \emph{map} pipeline, which takes as input a dataset of size $N$, the Shapley value can be computed in $O(N^2)$ time.
\end{corollary}


\subsection{Otpimizations for the 1-Nearest Neighbor Model} \label{sec:special-case-1nn}

We examine the special case when $K=1$. %This is a special case as it is much simpler to reason about, because
Since for each $v \in \mathcal{V}_{\mathcal{X}}$, there is always \emph{exactly} one tuple that is most similar to $t_{v}$. 
We now consider how to leverage this observation to construct the counting oracle.
%In an effort to construct the counting oracle for the $K=1$ case, 
Let $\phi_t(v)$ represent the event when $t$ is the top-$1$ tuple:
\begin{equation} \label{eq:top-1-condition-map-single}
\phi_t :=
p(t) \wedge
\bigwedge_{
    \substack{
        t' \in f(\mathcal{D}) \\
        \sigma(t') > \sigma(t)
    }
} \neg p(t').
\end{equation}
By definition, $\phi_t(v) := \mathrm{eval}_v (\phi_t)$. We can notice that, for \autoref{eq:top-1-condition-map-single} to be \emph{true} (i.e. for tuple $t$ to be the top-$1$), all tuples $t'$ where $\sigma(t') > \sigma(t)$ need to be \emph{absent} from the pipeline output. Hence, for a given value assignment, all provenance polynomials that control those tuples need to evaluate to $0$.

We now construct the function 
$$\phi_{t, t'}(v) := \phi_t(v[x_i \gets 0]) \wedge \phi_{t'}(v[x_i \gets 1]),$$
which is \emph{true} if $t$ is the top-$1$ tuple when $x_i \gets 0$ and $t'$ is the top-$1$ tuple when $x_i \gets 1$. This corresponds to the condition that our counting oracle counts models for. Expanding $\phi_{t, t'}(v)$, we obtain
\begin{equation} \label{eq:top-1-condition-map}
\resizebox{0.9\hsize}{!}{$
\phi_{t, t'} :=
\Big(
\neg x_i \wedge
p(t) \wedge
\bigwedge_{\substack{
    t'' \in f(\mathcal{D}) \\
    \sigma(t'') > \sigma(t)
}} \neg p(t'')
\Big)
\wedge
\Big(
x_i \wedge
p(t') \wedge
\bigwedge_{\substack{
    t'' \in f(\mathcal{D}) \\
    \sigma(t'') > \sigma(t')
}} \neg p(t'')
\Big).
$}
\end{equation}

Similarly, $\phi_{t, t'}(v) := \mathrm{eval}_v (\phi_{t, t'})$. It can only be \emph{true} if $p(t') \iff x_i$ and $\sigma(t) < \sigma(t')$. As a result, all provenance polynomials controlling tuples with a higher similarity score than that of $t$ need to evaluate to $0$. Therefore, the only polynomials that can be allowed to evaluate to $1$ are those corresponding to tuples with similarity score below $t$. Based on these observations, we can express the counting oracle for different types of ML pipelines.

%\medskip \noindent \textbf{Map Pipelines.} 
\inlinesection{Map Pipeline}
In a \emph{map} pipeline, the provenance polynomial for each tuple $t \in f(\mathcal{D})$ is defined by a single distinct variable $x \in \mathcal{X}$. Given our observation about $p(t') \iff x_i$, for a \emph{map} pipeline we can translate it to $p(t') = x_i$. Furthermore, if we observe the definition of the counting oracle from \autoref{eq:counting-oracle}, we can see that each oracle $\omega_{t, t'}$ counts the value assignments that result in support size $\alpha$ and label tally vectors $\gamma$ and $\gamma'$.

Given our observation about the provenance polynomials that are allowed to be set to $1$, we can easily construct an expression for counting valid value assignments. Namely, we have to choose exactly $\alpha$ variables out of the set $\{t'' \in \mathcal{D} \ : \ \sigma(t'') < \sigma(t) \}$, which corresponds to tuples with lower similarity than that of $t$. This can be constructed using a \emph{binomial coefficient}. Furthermore, when $K=1$, the label tally $\gamma$ is entirely determined by the top-$1$ tuple $t$. The same observation goes for $\gamma'$ and $t'$. To denote this, we define a constant $\Gamma_L$ that represents a tally vector with all values $0$ and only the value corresponding to label $L$ being set to $1$. We thus need to fix $\gamma$ to be equal to $\Gamma_{\ell (t)}$ (and the same for $\gamma'$). Finally, as we observed earlier, when computing $\omega_{t, t'}$ for $K=1$, the provenance polynomial of the tuple $t'$ must equal $x_i$. With these notions, we can define the counting oracle as
\begin{equation} 
\resizebox{0.9\hsize}{!}{$
\omega_{t, t'} (\alpha, \gamma, \gamma') = 
\binom{|\{t'' \in \mathcal{D} \ : \ \sigma(t'') < \sigma(t) \}|}{\alpha}
\mathbbm{1} \{ p(t')=x_i \}
\mathbbm{1} \{ \gamma = \Gamma_{\ell(t)} \}
\mathbbm{1} \{ \gamma' = \Gamma_{\ell(t')} \}.
$}
\label{eq:oracle-1nn}
\end{equation}
Note that we always assume $\binom{a}{b}=0$ for all $a < b$. We can prove the following corollary about \emph{map} pipelines:
\begin{corollary}
For the $1$-NN accuracy utility and a \emph{map} pipeline, which takes as input a dataset of size $N$, the Shapley value can be computed in $O(N \log N)$ time.
\end{corollary}

%\medskip \noindent \textbf{Fork Pipelines.} 
\inlinesection{Fork Pipeline}
As we have noted in the general case of $K$-NN, both \emph{map} and \emph{fork} pipelines result in polynomials made up of only one variable. The difference is that in \emph{map} pipelines each variable is associated with at most one polynomial, while in \emph{fork} pipelines it can be associated with multiple polynomials. However, when $K=1$, this difference vanishes when it comes to Shapley value computation:
\begin{corollary}
    For the $1$-NN accuracy utility and a \emph{fork} pipeline, which takes as input a dataset of size $N$, the Shapley value can be computed in $O(N \log N)$ time.
\end{corollary}
